Light quark masses in N_f = 2+1 lattice QCD with Wilson fermions

We present a lattice QCD determination of light quark masses with three sea-quark flavours ($N_f = 2+1$). Bare quark masses are known from PCAC relations in the framework of CLS lattice computations with a non-perturbatively improved Wilson-Clover action and a tree-level Symanzik improved gauge action. They are fully non-perturbatively improved, including the recently computed Symanzik counter-term $b_{\rm A} - b_{\rm P}$. The mass renormalisation at hadronic scales and the renormalisation group running over a wide range of scales are known non-perturbatively in the Schr\"odinger functional scheme. In the present paper we perform detailed extrapolations to the physical point, obtaining (for the four-flavour theory) $m_{u/d}(2{\rm GeV}) = 3.54(12)(9)$ MeV and $m_s(2{\rm GeV}) = 95.7(2.5)(2.4)$ MeV in the $\bar{MS}$ scheme. For the mass ratio we have $m_s/m_{u/d} = 27.0(1.0)(0.4)$. The RGI values in the three-flavour theory are $M_{u/d} = 4.70(15)(12)$ MeV and $M_s = 127.0(3.1)(3.2)$ MeV.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS

\newcommand{\parbreak}{\vskip 0.15cm}

% Abbreviations for environment tags
%\newcommand{\ba}{\begin{array}}
%\newcommand{\ea}{\end{array}}

% References
\newcommand{\req}[1]{Eq.~(\ref{#1})}
\newcommand{\res}[1]{Section~\ref{#1}}
\newcommand{\reapp}[1]{Appendix~\ref{#1}}
\newcommand{\rep}[1]{\cite{#1}}
\newcommand{\refig}[1]{Fig.~\ref{#1}}
\newcommand{\ret}[1]{Table~\ref{#1}}

% Miscellaneous symbols
\newcommand{\dif}{{\rm d}}
%\newcommand{\Tr}{{\rm Tr}}
%\newcommand{\tr}{{\rm tr}}
\newcommand{\Pf}{{\rm Pf}}
\newcommand{\Id}{\mathbf{1}}
\newcommand{\pexp}{\mbox{P} \, \mbox{exp}}
\newcommand{\Per}[1]{\mathbf{S}_{#1}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\ci}[1]{\boldsymbol{#1}}
\renewcommand{\Re}[1]{{\mathcal Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{{\mathcal Im}\left\{#1\right\}}
\newcommand{\Dslash}{\relax{\kern+.25em / \kern-.70em D}}
\newcommand{\Dwd}{D_{\rm\tiny W}}
\newcommand{\arcsinh}{\rm arcsinh}
\newcommand{\arccosh}{\rm arccosh}
\newcommand{\arctanh}{\rm arctanh}

% Numerical sets / Groups
\newcommand{\Real}{\relax{\mathsf{\Gamma\kern-.35em R}}}
\newcommand{\Int}{\relax{\mathsf{Z\kern-.40em Z}}}
\newcommand{\Ztwo}{Z_2}
%\newcommand{\Zf}{Z_4}
\newcommand{\ZN}{Z_{\NC}}
\newcommand{\ZTN}{Z_{2\NC}}
\newcommand{\UO}{\mbox{U}(1)}
\newcommand{\SUT}{\mbox{SU}(2)}
\newcommand{\UT}{\mbox{U}(2)}
\newcommand{\SUt}{\mbox{SU}(3)}
\newcommand{\Ut}{\mbox{U}(3)}
\newcommand{\SUN}{\mbox{SU}(\NC)}
\newcommand{\UN}{\mbox{U}(\NC)}
\newcommand{\SUQ}{\mbox{SU}(Q)}
\newcommand{\UQ}{\mbox{U}(Q)}
%\newcommand{\SU}{\mbox{SU}}
%\newcommand{\CF}{C_{\rm F}}

% Scriptstyle fractions
\newcommand{\half}{{\scriptstyle{{1\over 2}}}}
\newcommand{\third}{{\scriptstyle{{1\over 3}}}}
\newcommand{\quart}{{\scriptstyle{{1\over 4}}}}
\newcommand{\sixth}{{\scriptstyle{{1\over 6}}}}
\newcommand{\eighth}{{\scriptstyle{{1\over 8}}}}
\newcommand{\sixteenth}{{\scriptstyle{{1\over 16}}}}
\newcommand{\twth}{{\scriptstyle{{1\over 12}}}}
\newcommand{\thalf}{{\scriptstyle{{3\over 2}}}}
\newcommand{\fhalf}{{\scriptstyle{{5\over 2}}}}
\newcommand{\tthird}{{\scriptstyle{{2\over 3}}}}
\newcommand{\fthird}{{\scriptstyle{{5\over 3}}}}
\newcommand{\ihalf}{{\scriptstyle{{i\over 2}}}}
\newcommand{\iquart}{{\scriptstyle{{i\over 4}}}}
\newcommand{\oneovN}{{\scriptstyle{{1\over \NC}}}}

% Colours, flavours, susies
%\newcommand{\NC}{N_c}
\newcommand{\NC}{N}
\newcommand{\NF}{N_{\rm f}}
\newcommand{\NVAL}{N_{\rm val}}
\newcommand{\NSS}{{\cal N}}

\newcommand{\mav}{{m^{\rm av}}}
\newcommand{\Oav}{{O^{\rm av}}}


% Renormalisation schemes
%\newcommand{\MS}{{\rm MS}}
%\newcommand{\MSbar}{{\overline{\rm MS}}}
%\newcommand{\SF}{{\rm SF}}

% Renormalised, RGI and related quantities
%\newcommand{\gbar}{\kern1pt\overline{\kern-1pt g\kern-0pt}\kern1pt}
\newcommand{\gren}{g_{\rm R}}
\newcommand{\mbaref}[1]{m_{0, \rm #1}}
%\newcommand{\mbar}{\kern2pt\overline{\kern-1pt m\kern-1pt}\kern1pt}
\newcommand{\mbarf}[1]{\mbar_{\rm #1}}
\newcommand{\mren}[1]{m_{{\rm R} #1}}
\newcommand{\muren}[1]{\mu_{{\rm R} #1}}
\newcommand{\obar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\oren}[1]{#1_{\rm R}}
\newcommand{\corrbar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\corrren}[1]{#1_{\rm R}}
\newcommand{\lQCD}{\Lambda_{\rm\scriptscriptstyle QCD}}
\newcommand{\mrgi}{M}
\newcommand{\orgi}[1]{\hat #1}
%\newcommand{\orgi}[1]{#1_{\rm RGI}}
\newcommand{\msubt}{m_{\rm q}}
\newcommand{\mcrit}{m_{\rm cr}}
%\newcommand{\hopc}{\kappa_{\rm cr}}

\newcommand{\dstwo}{\scriptscriptstyle \Delta {\rm S} =2}

\newcommand{\oVA}[1]{#1_{\rm\scriptscriptstyle VA}}
\newcommand{\oAV}[1]{#1_{\rm\scriptscriptstyle AV}}
\newcommand{\oVV}[1]{#1_{\rm\scriptscriptstyle VV}}
\newcommand{\oAA}[1]{#1_{\rm\scriptscriptstyle AA}}

\newcommand{\oVApAV}[1]{#1_{\rm\scriptscriptstyle VA+AV}}
\newcommand{\oVAmAV}[1]{#1_{\rm\scriptscriptstyle VA-AV}}
\newcommand{\oSPpPS}[1]{#1_{\rm\scriptscriptstyle SP+PS}}
\newcommand{\oSPmPS}[1]{#1_{\rm\scriptscriptstyle SP-PS}}
\newcommand{\oVVpAA}[1]{#1_{\rm\scriptscriptstyle VV+AA}}
\newcommand{\oVVmAA}[1]{#1_{\rm\scriptscriptstyle VV-AA}}
\newcommand{\oSSpPP}[1]{#1_{\rm\scriptscriptstyle SS+PP}}
\newcommand{\oSSmPP}[1]{#1_{\rm\scriptscriptstyle SS-PP}}
\newcommand{\oTT}[1]{#1_{\rm\scriptscriptstyle TT}}
\newcommand{\oTtT}[1]{#1_{\rm\scriptscriptstyle T\tilde T}}
\newcommand{\oLL}[1]{#1_{\rm\scriptscriptstyle LL}}
\newcommand{\oRR}[1]{#1_{\rm\scriptscriptstyle RR}}
\newcommand{\oLR}[1]{#1_{\rm\scriptscriptstyle LR}}
\newcommand{\oRL}[1]{#1_{\rm\scriptscriptstyle RL}}

\newcommand{\oVApAVren}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt_{\rm\scriptscriptstyle VA+AV;s}}

% Correlation functions
\newcommand{\fX}{f_{\rm\scriptscriptstyle X}}
\newcommand{\fP}{f_{\rm\scriptscriptstyle P}}
\newcommand{\fS}{f_{\rm\scriptscriptstyle S}}
\newcommand{\fA}{f_{\rm\scriptscriptstyle A}}
\newcommand{\fV}{f_{\rm\scriptscriptstyle V}}
\newcommand{\kX}{k_{\rm\scriptscriptstyle X}}
\newcommand{\kA}{k_{\rm\scriptscriptstyle A}}
\newcommand{\kV}{k_{\rm\scriptscriptstyle V}}
\newcommand{\kT}{k_{\rm\scriptscriptstyle T}}
\newcommand{\hT}{h_{\rm\scriptscriptstyle T}}

\newcommand{\FY}{F_{\rm\scriptscriptstyle Y}}
\newcommand{\FVA}{F_{\rm\scriptscriptstyle VA}}
\newcommand{\FAV}{F_{\rm\scriptscriptstyle AV}}
\newcommand{\FVV}{F_{\rm\scriptscriptstyle VV}}
\newcommand{\FAA}{F_{\rm\scriptscriptstyle AA}}

\newcommand{\hVApAV}{h_{\rm\scriptscriptstyle VA+AV}}
\newcommand{\hVAmAV}{h_{\rm\scriptscriptstyle VAmAV}}
\newcommand{\hSPpPS}{h_{\rm\scriptscriptstyle SP+PS}}
\newcommand{\hSPmPS}{h_{\rm\scriptscriptstyle SP-PS}}
\newcommand{\hTtT}{h_{\rm\scriptscriptstyle T\tilde T}}

% Z's, SSF's et rel.
\newcommand{\Zm}{Z_{\rm m}}
\newcommand{\ZP}{Z_{\rm\scriptscriptstyle P}}
\newcommand{\ZS}{Z_{\rm\scriptscriptstyle S}}
\newcommand{\ZA}{Z_{\rm\scriptscriptstyle A}}
\newcommand{\ZV}{Z_{\rm\scriptscriptstyle V}}
\newcommand{\ZT}{Z_{\rm\scriptscriptstyle T}}
\newcommand{\ZVApAV}[1]{Z_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\ZVAmAV}[1]{Z_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\ZSPpPS}[1]{Z_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\ZSPmPS}[1]{Z_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\ZTtT}[1]{Z_{\rm\scriptscriptstyle T\tilde T #1}}
\newcommand{\ZtotVApAV}[1]{\mathcal{Z}_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\ZtotVAmAV}[1]{\mathcal{Z}_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\ZtotSPpPS}[1]{\mathcal{Z}_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\ZtotSPmPS}[1]{\mathcal{Z}_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\ZtotTtT}[1]{\mathcal{Z}_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\zbar}{\kern3pt\overline{\kern-2pt Z\kern-0pt}\kern1pt}
\newcommand{\zrgi}{\hat Z}
\newcommand{\zbarVApAV}[1]{\kern3pt\overline{\kern-2pt Z\kern-0pt}\kern1pt_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\zrgiVApAV}[1]{\hat Z_{\rm VA+AV #1}}

\newcommand{\sigmaP}{\sigma_{\rm\scriptscriptstyle P}}
\newcommand{\sigmaT}{\sigma_{\rm\scriptscriptstyle T}}
\newcommand{\SigmaP}{\Sigma_{\rm\scriptscriptstyle P}}
\newcommand{\SigmaT}{\Sigma_{\rm\scriptscriptstyle T}}

\newcommand{\sigVApAV}[1]{\sigma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\sigVAmAV}[1]{\sigma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\sigSPpPS}[1]{\sigma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\sigSPmPS}[1]{\sigma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\sigTtT}[1]{\sigma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\SigVApAV}[1]{\Sigma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\SigVAmAV}[1]{\Sigma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\SigSPpPS}[1]{\Sigma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\SigSPmPS}[1]{\Sigma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\SigTtT}[1]{\Sigma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\PISigVApAV}[1]{\tilde\Sigma_{\rm\scriptscriptstyle VA+AV #1}}

\newcommand{\UVApAV}[1]{U_{\rm\scriptscriptstyle VA+AV #1}}

\newcommand{\gamVApAV}[1]{\gamma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\gamVAmAV}[1]{\gamma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\gamSPpPS}[1]{\gamma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\gamSPmPS}[1]{\gamma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\gamTtT}[1]{\gamma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\lmax}{L_{\rm max}}
\newcommand{\lmin}{L_{\rm min}}
\newcommand{\mumax}{\mu_{\rm max}}
\newcommand{\mumin}{\mu_{\rm min}}

% O(a) improvement
%\newcommand{\Oa}{\mbox{O}(a)}
%\newcommand{\Oasq}{\mbox{O}(a^2)}
\newcommand{\Ogsqa}{\mbox{O}(g_0^2 a)}
\newcommand{\Ogqa}{\mbox{O}(g_0^4 a)}
\newcommand{\icsw}{c_{\rm sw}}
\newcommand{\ict}{c_{\rm t}}
\newcommand{\icttil}{\tilde c_{\rm t}}
\newcommand{\icP}{c_{\rm\scriptscriptstyle P}}
\newcommand{\icA}{c_{\rm\scriptscriptstyle A}}
\newcommand{\icT}{c_{\rm\scriptscriptstyle T}}
\newcommand{\icV}{c_{\rm\scriptscriptstyle V}}
\newcommand{\ibP}{b_{\rm\scriptscriptstyle P}}
\newcommand{\ibA}{b_{\rm\scriptscriptstyle A}}
\newcommand{\ibT}{b_{\rm\scriptscriptstyle T}}
\newcommand{\ibV}{b_{\rm\scriptscriptstyle V}}
\newcommand{\ibm}{b_{\rm m}}

% Boldface and calligraphic capitals
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% Boldface three-vectors and funny caps for momenta
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vzero}{\mathbf{0}}
%\newcommand{\ring}[1]{\mathaccent"7017 #1}

\newcommand{\scrA}{{\rm\scriptscriptstyle A}}
\newcommand{\scrP}{{\rm\scriptscriptstyle P}}
\newcommand{\scrV}{{\rm\scriptscriptstyle V}}

